Design Smells in Deep Learning Programs: An Empirical Study

Nowadays, we are witnessing an increasing adoption of Deep Learning (DL) based software systems in many industries. Designing a DL program requires constructing a deep neural network (DNN) and then training it on a dataset. This process requires that developers make multiple architectural (e.g., type, size, number, and order of layers) and configuration (e.g., optimizer, regularization methods, and activation functions) choices that affect the quality of the DL models, and consequently software quality. An under-specified or poorly-designed DL model may train successfully but is likely to perform poorly when deployed in production. Design smells in DL programs are poor design and-or configuration decisions taken during the development of DL components, that are likely to have a negative impact on the performance (i.e., prediction accuracy) and then quality of DL based software systems. In this paper, we present a catalogue of 8 design smells for a popular DL architecture, namely deep Feedforward Neural Networks which is widely employed in industrial applications. The design smells were identified through a review of the existing literature on DL design and a manual inspection of 659 DL programs with performance issues and design inefficiencies. The smells are specified by describing their context, consequences, and recommended refactorings. To provide empirical evidence on the relevance and perceived impact of the proposed design smells, we conducted a survey with 81 DL developers. In general, the developers perceived the proposed design smells as reflective of design or implementation problems, with agreement levels varying between 47\% and 68\%.

==> detection.tex <==
\section{Detection approach: \tool{}}\label{detection}
\subsection{Meta-modeling}
A DL program has different components. The core of each DL program is a DNN. For the sake of simplicity, we only consider the feedforward multilayer perceptron (MLP) architecture. Like other computational models, DNN attempts to find a mathematical mapping from the input into the output during a learning phase. Usually, a set of inputs and desired outputs (or targets) is provided for learning, which is called Dataset. Therefore, our meta-model includes three main parts: Architecture of DNN, Learner, and Data. Since we have used GTS for modeling DL programs, our proposed meta-model is represented by a type graph. The proposed type graph is illustrated in Figure \ref{fig:meta-model}. The node representing the \textbf{DL program} has three edges to \textbf{Architecture}, \textbf{Learner} and \textbf{Data} nodes indicating its main components. In the following, we describe the meta-model in detail. It should be noted that our aim of meta-modeling is the detection of faults in DL programs; therefore the most relevant components have been incorporated into the meta-model.\\
An architecture starts with the input layer, continues with some hidden layers and ends with the output layer. We have considered a distinctive node for the \textbf{InputLayer} because of its importance but all other successive layers are modelled as \textbf{Layer}. Each layer has a \textbf{size} indicating the number of neurons in that layer. There are specific properties among nodes that are modelled as edges. For example, \textbf{Architecture} starts by \textbf{Input Layer}, \textbf{Input Layer} is followed by other \textbf{Layer}s, each \textbf{Layer} may have next layers and each \textbf{Layer} has a \textbf{Type} as an attribute. There are different types for a layer in DL, e.g., dense, 1D and 2D convolution, pooling or data processing layers like flatten. There may be other attributes for a layer like \textbf{Bias}, \textbf{Weights}. An architecture ends with \textbf{Labels}, the desired outputs of DNN that are used to calculate the error of the network in \textbf{Loss} function. Actually, \textbf{Labels} is a part of \textbf{Data} associated with the DL program.\\
On the other hand, a model could be configured according to a DL program that has already been developed by a programmer. The source code of a DL program is converted to a model, which is an attributed graph. Dedicated convertors are programmed in \tool{} to convert a DL program written by different DL libraries to its model. The source code of a program is parsed to extract relevant information that is necessary to configure the model. The meta-model is generic enough to be independent of any specific DL library. Hence, we can have a model of a DL program that conforms to the meta-model; making possible further investigations on the model, such as verification. Apart from the work and analysis that are presented in the rest of this paper, we believe that this meta-model can be very useful to understand DL programs written by third parties. It will be helpful in understanding the development activities of DL practitioners; the way they write DL programs and the type of faults that they experience.

\begin{figure}
    \centerline{\includegraphics[width=\linewidth]{figs/meta-model.pdf}}
    \caption{The meta-model for DL models targeting deep FNNs.}
    \label{fig:meta-model}
\end{figure}

\subsection{Graph Transformations for Smell Detection}
In this paper, the meta-model is presented as a type graph and each model is a graph, instantiating the type graph. Each DL program is converted to a graph, as well. As a straightforward approach, graph transformations are chosen to implement the verification rules. Each verification rule is implemented as one or some graph transformations or graph processing operators. In fact, graph transformations are used to detect possible faults in a model, faults that are caused by violating the verification rules. Consequently, a transformation is applicable where the conditions of the corresponding rule are violated. In other words, if conditions of a verification rule are violated representing a fault in a model then the graph operation(s) of that rule will be applicable. Graph transformations are very flexible to find violation of some conditions in a graph. Recalling that a graph transformation \textit{r} is defined by a triplet of \textit{$(LHS_r, RHS_r, NAC_r)$}, a specific condition would be checked by finding a match of \textit{$LHS_r$} in the graph and/or the absence of \textit{$NAC_r$}. Once a graph operation is applied, i.e., detecting a fault in a part of graph, a specific fault code is added to the node or edge in which the violation occurred. This action is represented by the right hand-side of the rule \textit{$RHS_r$}.

\subsection{The tool} %\Foutse{give a name to the tool..different from NeuraLint to avoid confusion!}}
In this section, we describe our approach, \tool{} for detecting faults in DL programs. \tool{} is a model-based automated approach that performs a static analysis of a DL program to detect faults and design inefficiencies. Algorithm shows the pseudocode of \tool{}. The inputs are a DL program and a graph grammar, i.e., a set of graph transformations rules. As presented in Algorithm , \tool{} has three main steps: extract a graph from DL program, perform graph checking and generate a report from the resultant graph. At first, the DL program is modeled as a graph that conforms to the proposed meta-model, i.e., type graph. Then, a checking process runs to find bugs/issues in the model. This process attempts to apply rules to the graph and stops when further rule application becomes impossible. Then, \tool{} traverses this graph to generate a report for the user, containing a description of the faults and design issues found for each component. Except graph checking and graph transformations, all other parts of \tool{} are implemented in Python. We discuss details of each steps in the rest of this section.\\
%\begin{algorithm}[t]
%\KwIn{A DL program, \textit{program}, and \textit{rules} as a graph grammar}
%\KwOut{List of bugs or warnings to improve the program}
%\SetAlgoLined
% $graph \leftarrow{} \text{extractGraphFromProgram(\textit{program})}$\\
% $final \leftarrow{} \text{graphChecker(\textit{graph}, \textit{rules})}:$\\
% \begin{enumerate}
%  \item starting by \textit{graph}, apply enables rules.
%  \item apply enabled rules recursively.
%  \item terminate when further application of rules becomes impossible.
%  \item \Return \textit{final}.
% \end{enumerate}
% $report \leftarrow{} \text{extractReportFromGraph(\textit{final})}$\\
% \Return \textit{report}
% \caption{\tool}
% \label{algo:algo1}
 %%\vspace{-5pt}
%\end{algorithm}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/tool.pdf}
    \caption{The tool uses the DNN built by ML framework APIs to model a graph from DNN and then check the model to detect potential design smells.}
    \label{fig:tool}
\end{figure}

In our graph-based approach, a DL program is modeled by a graph instance conformed to the type graph, i.e., meta-model. To fulfill this primary step, we implement the graph generation relying on static code analysis that examines the source code and extracts the valuable code units and segments the information needed to instantiate the type graph's components. This provides a more holistic and semantic view of the analyzed DL program, that allows detecting faults related to either DL library's API misuse or DL algorithm implementation requirements. Hence, a specific graph generator should be implemented for each supported DL library. Without loss of its generality, \tool{} currently supports DL programs written using TensorFlow and Keras as two well-known and popular libraries. It should be noted that \tool{} can be extended to work for other DL libraries, as well. In the following, we describe steps of modeling of DL programs as attributed graphs.

The verification rules are implemented as graph transformations to process and verify the graph. Each graph transformation applies to the graph if conditions of the rule are violated. Once the DL source code is modeled as a graph, the violations of rules can be detected with a graph transformation tool that executes the sequence of rules over the model of the DL program. In this paper, we have used the GROOVE toolset \cite{rensink2004groove} to perform graph operations. GROOVE is a tool for implementing, simulating, and analysis of graph transformation systems. It is capable of exploring recursively and collecting all possible rule applications over a host (start) graph. This is referred to as the exploration of the state space of a graph grammar. GROOVE explores the state space by applying a slightly modified version of standard graph traversal algorithms, like depth-first search (DFS) or breadth-first search (BFS). Furthermore, it has a graphical interface for editing graphs and rules, and for exploring and visualising the GTS which could be called via command line, as well. The output of GROOVE is called the final graph on which no further rule application is possible. For more information about GROOVE’s internal mechanism and its capabilities for modeling and simulating GTS, the interested reader may refer to \cite{ghamarian2012modelling}.\\

\section{Evaluation}\label{evaluation}
\subsection{Evaluated programs}
We manually inspected, for each type of bug, the top-10 relevant SO posts (i.e., according to built-in SO relevance criterion) mentioning one or more of its associated keywords. We consider SO posts, containing full code script or code snippets that are related to one or multiple bugs belonging to the above-mentioned categories.

\subsection{Results}

==> table-1.tex <==
\begin{table*}
\caption{Validation results: Perceived relevance of the 8 design smells \Foutse{can you bold or colour the cells of the ones with more than 50\% agreement?}}
\label{validationTable}
%\resizebox{.99\textwidth}{!}{
\begin{center}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|}
\hline

\multirow{3}{*}{\textbf{Design Smells}} & \multicolumn{5}{c|}{\textbf{Responses}}\\
& Strongly & \multirow{2}{*}{Disagree} & \multirow{2}{*}{Borderline} & \multirow{2}{*}{Agree} & Strongly \\
& disagree & & & & agree \\
\hline
\hline
Non-expanding feature map & 6\% & 15\% & 16\% & 46\% & 17\% \\

\hline
Losing local correlation & 12\% & 15\% & 24\% & 32\% & 17\% \\

\hline
Heterogeneous blocks of CNNs & 4\% & 6\% & 26\% & 42\% & 22\% \\

\hline
Too much down-sampling & 9\% & 14\% & 22\% & 36\% & 17\% \\

\hline
Non-dominating down-sampling & 7\% & 19\% & 18\% & 34\% & 22\% \\

\hline
Useless Dropout & 7\% & 14\% & 23\% & 31\% & 25\% \\

\hline
Bias With Batchnorm & 11\% & 9\% & 33\% & 31\% & 16\% \\

\hline
Non-representative Statistics Estimation & 5\% & 10\% & 17\% & 33\% & 35\% \\

\hline
\end{tabular}}
\end{center}
\label{table:table-results-1}
%}
\end{table*}

==> table-2.tex <==
\begin{table}[t]
\caption{Survey results about a detection tool}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Questions}} & \multicolumn{2}{|c|}{\textbf{Responses}} \\
\cline{2-3} 
 & \textbf{Yes}& \textbf{No} \\
\hline
\hline
Can a detection tool for design smells be helpful? & 90\% & 10\% \\
\hline
Do you use such a tool? & 86\% & 14\%\\
\hline
\end{tabular}}
\label{table2}
\end{center}
\end{table}
